Canonical extensions of lattices are more than perfect

In \cite{CGH15} we introduced TiRS graphs and TiRS frames to create a new natural setting for duals of canonical extensions of lattices. In this continuation of \cite{CGH15} we answer Problem 2 from there by characterising the perfect lattices that are dual to TiRS frames (and hence TiRS graphs). We introduce a new subclass of perfect lattices called PTi lattices and show that the canonical extensions of lattices are PTi lattices, and so are `more' than just perfect lattices. We introduce morphisms of TiRS structures and put our correspondence between TiRS graphs and TiRS frames from \cite{CGH15} into a full categorical framework. We illustrate our correspondences between classes of perfects lattices and classes of TiRS graphs by examples.

==> lat.tex <==
%%AMSTEX version of lat.tex


% as of dec 11 95

%lat.tex July 15, 1995

%last update November 18, 1995
%  flaps added

%basic lattices and ordered sets
% extended to include various diagrams from ILO and some other
% useful extant diagrams
%September 16, 1995
  %chains added

%%  catalogue
%    tiny           small          large      

%                 \chainthreeii                 3 element chain  $\ch 3$
%                 \nfiveii       \nfiveiii      $N_5$
%  \tmthree       \mthreeii      \mthreeiii     $M_3$
%                                \mfouriii      $M_4$
%  \ttwosq        \twosqii       \twosqiii      $\ch 2^2$
%  \ttwothree     \twothreeii                   $\ch 2 \times \ch 3$
%                 \threetwoii    \threetwoiii   $\ch 3 \times \ch 2$
%  \tthreesq      \threesqii     \threesqiii    $\ch 3^2$
%                 \threefourii   \threefouriii  $\ch 3 \times \ch 4$
%  \tfoursq                                     $\ch 4^2$
%  \tcube         \cubeii        \cubeiii       cube $\ch 2^3$
%                            with associated \rflap \lflap for \cubeiii
%  \tskewcube     \skewcube                     skew cube
%  with associated \trskewflap  \rlskewflap 
%                  \rskewflap  \lskewflap
%
%                 \2sq, \1sqmkii, \1sqmkiii   3 versions of  $\ch 2^4$
%                                             [ILO Figure 1.10]
%                  \en                        N
%                  \tree                      labelled binary tree 
%                                             [ILO 1.6]
%                 \fd3                        free 0,1 dl on 3 gens
%                                             [ILO 8.5]
%                 \mthreethree                $M_{3,3}$ [ILO 6.5]
%                 \fivesixteen                [ILO 5.16]
%                 \bfly                       linear sum of 2 2-el antichains
%                 \tower                      linear sum of s 2 el antichains [lavelled]

%  chii
%  chiii
%\chiv
%\chv
%\chvi

\def\schainii{\hbox{
	\point 0 0 
	\point 0 1
	\vline 0 0 1
}}

\def\schainiii{\hbox{
	\point 0 0 
	\point 0 1
	\point 0 2
	\vline 0 0 1
	\vline 0 1 1
}}

\def\chainii{\hbox{
  \point 0 0
  \point 0 2
  \vline 0 0 2
}}

\def\chainiii{\hbox{
  \point 0 0
  \point 0 2
\point 0 4
  \vline 0 0 2
  \vline 0 2 2
}}
                  

\def\chainiv{\hbox{
  \point 0 0
  \point 0 2
\point 0 4
\point 0 6

  \vline 0 0 2
  \vline 0 2 2
  \vline 0 4 2

}}                

\def\chainv{\hbox{
  \point 0 0
  \point 0 2
\point 0 4
\point 0 6
\point 0 8


  \vline 0 0 2
  \vline 0 2 2
  \vline 0 4 2
  \vline 0 6 2


}}                



\def\chainvi{\hbox{
  \point 0 0
  \point 0 2
\point 0 4
\point 0 6
\point 0 8
\point 0 10



  \vline 0 0 2
  \vline 0 2 2
  \vline 0 4 2
  \vline 0 6 2
  \vline 0 8 2
}}



\def\chii{\hbox{
  \point 0 0
  \point 0 2
  \vline 0 0 2
}}


\def\chii{\hbox{
  \point 0 0
  \point 0 2
  \vline 0 0 2
}}


\def\rflap{\hbox{
\point 0 0
\point 3 3
\point 0 3
\point 3 6
\slps 0 0 3
\slps 0 3 3
\vline 0 0 3
\vline 3 3 3
}}               
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\lflap{\hbox{
\point 0 0
\point -3 3
\point 0 3
\point -3 6
\slms -3 3 3
\slms -3 6 3
\vline 0 0 3
\vline -3 3 3
}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\rskewflap{\hbox{
\point 0 0 
\point 4 3
\point 0 3
\point 4 6
\sssslpsss 0 0 4
\sssslpsss 0 3 4
\vline 0 0 3
\vline 4 3 3
}}                   

\def\lskewflap{\hbox{
\point 0 0 
\point -4 3
\point 0 3
\point -4 6
\sssslmsss -4 3 4
\sssslmsss -4 6 4
\vline 0 0 3
\vline -4 3 3
}}                   

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\tlskewflap{\hbox{
\point 0 0 
\point -1 2
\point 0 2
\point -1 4
\slmss -1 2 2
\slmss -1 4 2
\vline 0 0 2
\vline -1 2 2
}}                   


\def\trskewflap{\hbox{
\point 0 0 
\point 1 2
\point 0 2
\point 1 4
\slpss 0 0 2
\slpss 0 2 2
\vline 0 0 2
\vline 1 2 2
}}                   


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%                
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


                


\def\skewcube{\hbox{
\point 0 0 
\point 4 3
\point 0 3
\point -2 3
\point -2 6
\point 4 6
\point 2 6
\point 2 9
\sssslpsss 0 0 4
\sssslpsss 0 3 4
\sssslpsss -2 3 4
\sssslpsss -2 6 4
\sslmsss -2 3 3
\sslmsss -2 6 3
\sslmsss 2 6 3
\sslmsss 2 9  3
\vline 0 0 3
\vline 4 3 3
\vline 2 6 3
\vline -2 3 3
}}                  
                    
                    
\def\nfiveii{\hbox{
\point 0 0
\point 2 2
\point 0 4
\point -2 1.33333
\point -2 2.66666 
\slps 0 0 2
\slms 0 4 2
\ssslpss -2 2.66666 2
\vline  -2 1.3333  1.3333 
\ssslmss -2  1.3333 2
}}
                    
\def\nfiveiii{\hbox{
\point 0 0
\point 0 6
\point -2 2
\point -2 4
\point 2 3
\vline -2 2 2
\slms -2 2 2
\slps -2 4 2
\sslpsss 0 0 3
\sslmsss 0 6 3
}}

\def\tmthree{\hbox{
 \point 0 0
\point 1.5 1.5
\point -1.5 1.5
\point 0 1.5
\point 0 3
\tlinep 0 0
\tlinem 0 0
  \tlinem 1.5 1.5
\tlinep -1.5 1.5
\tvline 0 0
\tvline 0 1.5
}}



\def\ttwosq{\hbox{
   \point 0 0
    \point 1.5 1.5
   \point -1.5 1.5
  \point 0 3
  \tlinep 0 0
  \tlinep -1.5 1.5
  \tlinem 1.5 1.5
 \tlinem 0 0
  }}                   



\def\ttwosqsdots{\hbox{\scircles
\put -.1 -.1 {\hbox{
   \put 0 0  {$\sspoint$} 
    \put 1.5 1.5  {$\sspoint$}
   \put  -1.5 1.5  {$\sspoint$}    
  \put 0 3   {$\sspoint$} 
  }}              
}}

\def\tfoursq{\hbox{
   \point 0 0
    \point 1.5 1.5
   \point -1.5 1.5
  \point 0 3
   \point 3 3
   \point -3 3
    \point -1.5 4.5
    \point 1.5 4.5
     \point 0 6
    \tlinep  1.5 1.5
    \tlinep  0 3
    \tlinep -3 3
    \tlinep -1.5 4.5
    \tlinem  -1.5 1.5
     \tlinem 0 3
     \tlinem 1.5 4.5
     \tlinem 3 3
  \tlinep 0 0
  \tlinep -1.5 1.5
  \tlinem 1.5 1.5
 \tlinem 0 0
\point 4.5 4.5
\point -4.5 4.5
\point 3 6
\point -3 6
\point 1.5 7.5
\point -1.5 7.5
\point 0 9
\tlinep 3 3
\tlinep 1.5 4.5
\tlinep 0 6
\tlinep -1.5 7.5
\tlinep -3 6
\tlinep -4.5 4.5
\tlinem  4.5 4.5
\tlinem 3 6
\tlinem 1.5 7.5
\tlinem -3 3
\tlinem -1.5 4.5
\tlinem 0 6
  }} 

\def\tthreesq{\hbox{
   \point 0 0
    \point 1.5 1.5
   \point -1.5 1.5
  \point 0 3
   \point 3 3
   \point -3 3
    \point -1.5 4.5
    \point 1.5 4.5
     \point 0 6
    \tlinep  1.5 1.5
    \tlinep  0 3
    \tlinep -3 3
    \tlinep -1.5 4.5
    \tlinem  -1.5 1.5
     \tlinem 0 3
     \tlinem 1.5 4.5
     \tlinem 3 3
  \tlinep 0 0
  \tlinep -1.5 1.5
  \tlinem 1.5 1.5
 \tlinem 0 0
}}

\def\tthreesqnine{\hbox{
   \point 0 0
    \point 1.5 1.5
   \point -1.5 1.5
  \point 0 3
   \point 3 3
   \point -3 3
    \point -1.5 4.5
    \point 1.5 4.5
     \point 0 6
     
     \point -4.5 4.5
     \point -3 6 
     \point -1.5 7.5 
     \point 0 9 
     \point 1.5 7.5
     \point 3 6 
     \point 4.5 4.5
     
     \tlinep -4.5 4.5
     \tlinep -3 6 
     \tlinep -1.5 7.5 
     \tlinep 0 6 
     \tlinep 1.5 4.5 
     \tlinep 3 3
     
     \tlinem -3 3 
     \tlinem -1.5 4.5 
     \tlinem 0 6 
     \tlinem 1.5 7.5
     \tlinem 3 6
     \tlinem 4.5 4.5
     
    \tlinep  1.5 1.5
    \tlinep  0 3
    \tlinep -3 3
    \tlinep -1.5 4.5
    \tlinem  -1.5 1.5
     \tlinem 0 3
     \tlinem 1.5 4.5
     \tlinem 3 3
  \tlinep 0 0
  \tlinep -1.5 1.5
  \tlinem 1.5 1.5
 \tlinem 0 0
}}


        
\def\sspoint{\scriptscriptstyle{\bullet}}                   

\def\tthreesqsdots{\hbox{\scircles
\putt -.1 -.1 {\hbox{
\putt 0 0    {$\sspoint$}  
 \putt 1.5 1.5  {$\sspoint$}    
 \putt -1.5 1.5  {$\sspoint$} 
\putt  0 3  {$\sspoint$} 
\putt 3 3  {$\sspoint$}  
 \putt -3 3   {$\sspoint$} 
\putt  -1.5 4.5  {$\sspoint$} 
\putt 1.5 4.5  {$\sspoint$} 
\putt 0 6   {$\sspoint$} 
}}
}}



\def\twosqii{\hbox{
\point 0 0
\point 2 2
\point -2 2
\point 0 4
\slps 0 0 2
\slms -2 2 2
\slps -2 2 2
\slms 0 4 2
}}                 

\def\mthreeii{\hbox{
\point 0 0
\point 0 2
\point 0 4
\point 2 2
\point -2 2
\slps 0 0 2
\slps -2 2 2
\slms -2 2 2
\slms 0 4  2
\vline 0 0 2
\vline 0 2 2
}}

\def\mthreeiii{\hbox{
\point 0 0
\point 0 3
\point 0 6
\point 3 3
\point -3 3
\slps 0 0 3
\slps -3 3 3
\slms -3 3 3
\slms 0 6 3
\vline 0 0 3
\vline 0 3 3
}}



\def\threesqii{\hbox{\point  0 0
\point 2 2
\point -2 2
\point -4 4
\point 0 4
\point 4 4
\point -2 6
\point 2 6
\point 0 8
\slps  0 0 2   
\slps  2 2 2
\slps  -2 2 2
\slps  -4 4 2
\slps  0 4 2
\slps  -2 6 2
\slms  -2 2   2
\slms  0 4   2
\slms  2 6 2
\slms  -4 4   2
\slms  -2 6    2
\slms  0 8  2
}}                              

                                
\def\threefourii{\hbox{
\point  0 0
\point 2 2
\point -2 2
\point -4 4
\point -6 6
\point -4 8
\point -2 10
\slps -6 6 2
\slps -4 8 2
\slms -6 6 2
\slms -4 8 2
\slms -2 10 2
\point 0 4
\point 4 4
\point -2 6
\point 2 6
\point 0 8
\slps  0 0 2   
\slps  2 2 2
\slps  -2 2 2
\slps  -4 4 2
\slps  0 4 2
\slps  -2 6 2
\slms  -2 2   2
\slms  0 4   2
\slms  2 6 2
\slms  -4 4   2
\slms  -2 6    2
\slms  0 8  2
}}
                                
\def\threesqiii{\hbox{\point  0 0
\point 3 3
\point -3 3
\point -6 6
\point 0 6
\point 6 6
\point -3 9
\point 3 9
\point 0 12
\slps  0 0 3   
\slps  3 3 3
\slps  -3 3 3
\slps  -6 6 3
\slps  0 6 3
\slps  -3 9 3
\slms  -3 3   3
\slms  0 6   3
\slms  3 9 3
\slms  -6 6   3
\slms  -3 9    3
\slms  0 12  3
}}
                                 
\def\threefouriii{\hbox{
\point  0 0
\point -9 9
\point -6 12
\point -3 15
\slps -9 9 3
\slps -6 12 3
\slms -9 9 3
\slms -6 12 3
\slms -3 15 3
\point 3 3
\point -3 3
\point -6 6
\point 0 6
\point 6 6
\point -3 9
\point 3 9
\point 0 12
\slps  0 0 3   
\slps  3 3 3
\slps  -3 3 3
\slps  -6 6 3
\slps  0 6 3
\slps  -3 9 3
\slms  -3 3 3
\slms  0 6 3
\slms  3 9 3
\slms  -6 6 3
\slms  -3 9 3
\slms  0 12 3
}}

                                 


\def\twothreeii{\hbox{
\point  0 0
\point 2 2
\point 4 4
\point -2 2
\point 0 4
\point 2 6 

\slps 0 0 2
\slps 2 2 2
\slps -2 2 2
\slps  0 4 2

\slms -2 2 2
\slms 0 4 2
\slms 2 6 2
}}

\def\ttwothree{\hbox{
\point  0 0
\point 1.5 1.5
\point 3  3
\point -1.5 1.5
\point 0 3
\point 1.5 4.5

\tlinep 0 0 
\tlinep 1.5 1.5
\tlinep -1.5 1.5 
\tlinep  0  3 

\tlinem 0 0 
\tlinem 1.5   1.5
\tlinem 3 3 
}}


                            
\def\ttwothreesdots{\hbox{\scircles
\put -.1 -,1  {\hbox{ 
\put  0 0   {$\sspoint$}
\put 1.5 1.5 {$\sspoint$}
\put 3  3     {$\sspoint$}
\put -1.5 1.5   {$\sspoint$}
\put 0 3       {$\sspoint$}
\put 1.5 4.5   {$\sspoint$}
}}
}}






\def\cubeiii{\hbox{
\point 0 0
\point 0 3
\point -3 3
\point 3 3
\point 0 6
\point -3 6
\point  3 6
\point  0 9
\slps 0 0 3
\slps 0 3 3
\slps -3 3 3
\slps -3 6 3
\slms -3 3 3
\slms -3 6 3
\slms 0 6 3
\slms 0 9 3 
\vline 0 0 3
\vline -3 3 3
\vline 3 3 3
\vline 0 6 3
}}
                   
\def\cubeii{\hbox{ 
\point 0 0
\point 0 2
\point -2 2
\point 2 2
\point 0 4
\point -2 4
\point  2 4
\point  0 6
\slps 0 0 2
\slps 0 2 2
\slps -2 2 2
\slps -2 4 2
\slms -2 2 2
\slms -2 4 2
\slms 0 4 2
\slms 0 6 2 
\vline 0 0 2
\vline -2 2 2
\vline 2 2 2
\vline 0 4 2
}}

\def\threetwoii{\hbox{
\point 0 0
\point -2 2
\point -4 4
\point 2 2
\point 0 4
\point -2 6
\slps  0 0 2
\slps -2 2 2
\slps  -4 4 2
\slms -2 2 2
\slms -4 4 2
\slms 0 4 2
\slms -2 6 2
}}                            

\def\threetwoiii{\hbox{
\point 0 0
\point -3 3
\point -6 6
\point 3 3
\point 0 6
\point -3 9
\slps  0 0 3
\slps -3 3 3
\slps  -6 6 3
\slms -3 3 3
\slms -6 6 3
\slms 0 6 3
\slms -3 9 3
}}

\def\tcube{\hbox{ 
     \point 0 0
     \point -1.5 1.5
     \point 1.5 1.5
     \point 0 1.5
     \point -1.5 3
     \point 0 3
     \point 1.5 3
     \point 0 4.5
     \tvline 0 0
     \tvline -1.5 1.5
     \tvline 1.5 1.5
     \tvline 0 3
     \tlinep 0 0
     \tlinep 0 1.5
     \tlinep -1.5 1.5
     \tlinep -1.5 3
     \tlinem 0 0 
     \tlinem 0 1.5
     \tlinem 1.5 1.5
     \tlinem 1.5 3
      }}


\def\fivesixteen{\hbox{\multiput 0 0 0 2 6 {\hbox{\point 0 0 }} %5.16
                  \multiput 0 0 0 2 5 {\hbox{\vline 0 0 2 }}
                  \point -2 2
                  \point -2 4
                  \point -2 8
                  \point 2 2
                  \point 2 6 
                  \vline -2 2 2 
                  \vline -2 4 4
                  \vline 2 2 4
                  \slps 0 0 2
                  \slps -2 2 2
                  \slps -2 4 2
                  \slps -2 8 2
                  \slms -2 2 2
                  \slms 0 4 2
                   \slms 0 8 2
}}
\def\twosqiii{\hbox{
\point 0 0
\point 3 3
\point -3 3
\point 0 6
\slps 0 0 3
\slms -3 3 3
\slps -3 3 3
\slms 0 6 3
}}                  
\def\chainthreeii{\hbox{ \point 0 0
                          \point 0 2
                         \point 0 4
                         \vline 0 0 2
                         \vline 0 2 2
                           }}
\def\mfouriii{\hbox{\point 0 0
                    \point 0 6
                    \point 2 3
                    \point 4 3
                    \point -2 3
                   \point -4 3
                   \sssslpsss 0 0 4
                   \sssslpsss -4 3 4
                   \sssslmsss -4 3 4
                   \sssslmsss 0 6 4
                    \sslpsss 0 0 3
                    \sslpsss -2 3 3
                    \sslmsss -2 3 3
                   \sslmsss 0 6 3
               }}


\def\mfouriii{\hbox{\putt 0 0 {\twosqiii}
                    \point 1 3
                    \point -1 3
                    \slpsss 0 0 3
                    \slpsss -1 3 3
                    \slmsss -1 3 3
                   \slmsss 0 6 3
               }}

\def\tskewcube{
 {\hbox{
 \point  0 0
 \point  -1 2
 \point  2 2
 \point  0 2
 \point  -1 4
 \point  1 4
 \point 2 4
 \point  1 6
 \slps  0 0 2       
 \slps  0 2 2       
 \slps  -1 2 2       
 \slps  -1 4 2       
 \slmss  -1 2 2        
 \slmss  -1 4 2       
 \slmss  1 6 2       
 \slmss  1 4 2       
 \vline 0 0 2
\vline -1 2 2
\vline 2 2 2
\vline 1 4 2
}}
}              

%symmetric 2^4
\def\twosq{\hbox{
  \putt 0 0 {\twosqii}
  \putt 6 3 {\twosqii}  
\putt -6 3 {\twosqii}
\putt 0 6 {\twosqii}
\sslps 0 0 6
\sslps -2 2 6
\sslps 2 2 6
\sslps 0 4 6
\sslms 0 6  6
\sslms  2 8 6
\sslms  -2 8 6
\sslms  0 10 6
\sslms  -4 5 6
\sslms  -6 3 6
\sslms   -8 5 6
\sslms   -6 7 6
\sslps  -4 5 6
\sslps  -6 3 6
\sslps   -8 5 6
\sslps   -6 7 6
}}


\def\twosqmkii{\hbox{
       \point 0 0
      \point -1 2
       \point 1 2
       \point 3 2
       \point -3 2
          \point -1 4
       \point 1  4
       \point 3 4
       \point -3 4
        \point -5 4
        \point 5  4
        \point 1  6
       \point 3 6
       \point -3  6
        \point -1  6           
      \point 0 8
       \vline 1  2 2
        \vline -3 2 2
       \vline  3 2 2
       \vline  3 4 2
       \vline  -3 4 2
       \vline  -1 4 2
        \slpss 0 0 2
         \slpss -1 6 2
          \slmss 0 8 2
           \slmss -1 2 2
          \ssslpss 0 0 3
         \ssslmss -3  2 3
         \ssslpss -3 6 3
          \ssslmss 0 8 3
          \linep 3  2 2
           \linep -5 4 2
         \linem -3 2 2
          \linem 5  4 2
          \sslps 1 2 4
          \sslps -1 2 4
         \sslps -5 4 4
         \sslps -3 4 4
         \sslms -5 4 4
         \sslms -3 4 4
          \sslms -1  4 4
          \sslms -3 6  4
          \sslms -1 6 4
          \sslms 1 6 4
           \linep -3 2 2
           \linep -1 4 2 
          \linep -1 2 2
          \linep 1 4 2
}}

\def\twosqmkiii{\hbox{
        \point 0 0 
        \point -3 1.2
       \point 3 1.2
       \point 1.2 3
        \point -1.2 3
         \point 0 2.4
       \point 4.2 4.2
       \point -4.2 4.2
        \point 1.8 4.2
         \point -1.8 4.2
        \point 1.2 5.4
        \point -1.2 5.4
       \point 0 6
      \point 3 7.2
      \point -3 7.2
     \point 0 8.4
       \svlpss 0 0 3
       \svlpss 1.2 3 3
      \svlpss -1.2 3 3
      \svlpss -3 1.2 3
     \svlpss -1.8 4.2 3
     \svlpss -4.2 4.2 3
      \svlpss 0 6 3
      \svlpss -3 7.2 3
      \sslpsv 0 0 3
     \sslpsv 3 1.2 3
     \sslpsv 1.8 4.2 3
    \sslpsv 0 2.4 3
    \sslpsv -1.2 3 3
     \sslpsv -4.2 4.2 3
     \sslpsv -1.2 5.4 3
      \sslpsv -3 1.2  3
     \sslmsv -1.2 3 3
    \sslmsv 1.8 4.2 3
     \sslmsv 3 7.2 3
    \sslmsv 0 8.4 3
      \svlmss -1.8 4.2 3
     \sslmsv -1.2 5.4 3
      \sslmsv -4.2 4.2 3
       \sslmsv -3 7.2 3
    \sslmsv 0 6 3
     \svlmss -3 1.2 3
    \svlmss -4.2 4.2 3
    \svlmss -3 7.2 3
   \svlmss -1.2 5.4 3
  \svlmss 0 8.4 3
  \svlmss 1.2 5.4 3
   \svlmss 0 2.4 3
  \svlmss -1.2  5.4 3
}}

\def\en{\hbox{
      \point -1.5   0
     \point -1.5 3
     \point 1.5 0
   \point 1.5 3
    \vline -1.5 0 3
\vline 1.5 0 3
 \slms -1.5 3 3
}}

  \def\tree{\hbox{
          \point 0 0
        \point -6 2
         \point 6 2
         \point -9 4
         \point -3 4
         \point 3 4
        \point 9 4
        \point -10 6
       \point -8 6
       \point -4 6
       \point -2 6
        \point 2 6
      \point 4 6
       \point 8 6
       \point 10 6
      \ssslps 0 0  6
      \ssslms -6 2 6
       \ssslpss -6 2 3
       \ssslmss -9 4 3
        \ssslmss 3 4 3
       \ssslpss 6 2 3
       \slpss -9 4 2
       \slpss -3 4 2             
       \slpss 3 4 2
       \slpss 9 4 2
      \slmss -10 6 2
      \slmss -4 6 2
      \slmss 2 6 2
      \slmss 8 6 2
      \labelr 0 -0.5 {{}_\emptyset}
      \labelr 6 2 {{}_1}
      \labell -7 2 {{}_0}
     \labelr -9 4 {{}_{00}}
\labelr -3 4 {{}_{01}}
 \labelr 3 4 {{}_{10}}
\labelr 9 4 {{}_{11}}
\putt -10.8 6.6 {${}_{000}$}
\putt -8.8 6.6 {${}_{001}$}
\putt -4.8 6.6 {${}_{010}$}
\putt -2.8 6.6 {${}_{011}$}
\putt 1.2 6.6 {${}_{100}$}
\putt 3.2 6.6 {${}_{101}$}
\putt 7.2 6.6 {${}_{110}$}
\putt 9.2 6.6 {${}_{111}$}
}}

\def\fd3{\hbox{
          \putt 0 1.5  {\tcube}
          \putt 0 6 {\tcube}
          \point 0 0
          \point 0 12
          \tvline 0 0 
          \tvline 0 10.5
          \point 1.5 6
          \point 3 6
         \point -3 6
          \tlinep  0 4.5
          \tlinep 1.5 4.5
          \tlinep -3 6
         \tlinem 1.5 6
         \tlinem 3 6
        \tlinem -1.5 4.5
      }}

\def\mthreethree{\hbox{\putt 0 0 {\mthreeii}
                 \putt 2 2 {\mthreeii}
                 }}

\def\bfly{\hbox{
  \point -1 0
 \point 1 0
\point -1 2
\point 1 2
\vline -1 0 2
\vline 1 0 2
\slps -1 0 2
\slms -1 2 2
}}


\def\tower{\hbox{
\putt 0 0 {\bfly}
\putt 0 2 {\bfly}
\putt 0 8 {\bfly}
\tvline -1 6.5
\tvline 1 6.5
\tvline -1 4
\tvline 1 4
\putt -1.2 6.1 {$\cdot$}
\putt -1.2 5.8 {$\cdot$}
\putt -1.2 5.5 {$\cdot$}
\putt 0.8 6.1 {$\cdot$}
\putt 0.8 5.8 {$\cdot$}
\putt 0.8 5.5 {$\cdot$}
\labelr -3 0 {x_1^1}
\labelr -3 2 {x_2^1}
\labelr -3 4 {x_3^1}
\labelr -3.7 8 {x_{s-1}^1}
\labelr -3 10 {x_{s}^1}
\labelr 1 0 {x_1^2}
\labelr 1 2 {x_2^2}
\labelr 1 4 {x_3^2}
\labelr 1 8 {x_{s-1}^2}
\labelr 1 10 {x_{s}^2}
}}

\def\urcdots{\hbox{
\putt 0 0 {$\cdot$}
\putt 0.5 0.5 {$\cdot$}
\putt 1 1 {$\cdot$}
\putt 1.5 1.5 {$\cdot$}
\putt 2 2 {$\cdot$}
\putt 2.5 2.5 {$\cdot$}
}}

\def\drcdots{\hbox{
\putt -0.1 -0.1 {\hbox{
\putt 0 0 {$\cdot$}
\putt 0.5 -0.5 {$\cdot$}
\putt 1 -1 {$\cdot$}
\putt 1.5 -1.5 {$\cdot$}
\putt 2 -2 {$\cdot$}
\putt 2.5 -2.5 {$\cdot$}
}}
}}

\def\ur1cdots{\hbox{
\putt 0 0 {$\cdot$}
\putt 1 1 {$\cdot$}
\putt 2 2 {$\cdot$}
}}

\def\dr1cdots{\hbox{
\putt -0.1 -0.1 {\hbox{
\putt 0 0 {$\cdot$}
\putt 1 -1 {$\cdot$}
\putt 2 -2 {$\cdot$}
}}
}}


\def\dlcdots{\hbox{
\putt 0 0 {\hbox{
\putt 0 0 {$\cdot$}
\putt -0.5 -0.5 {$\cdot$}
\putt -1 -1 {$\cdot$}
\putt -1.5 -1.5 {$\cdot$}
\putt -2 -2 {$\cdot$}
\putt -2.5 -2.5 {$\cdot$}
}}
}}

\def\dl1cdots{\hbox{
\putt 0 0 {$\cdot$}
\putt -1 -1 {$\cdot$}
\putt -2 -2 {$\cdot$}
}}


\def\ulcdots{\hbox{
\putt -0.2 -0.2 {\hbox{
\putt 0 0 {$\cdot$}
\putt -0.5 0.5 {$\cdot$}
\putt -1 1 {$\cdot$}
\putt -1.5 1.5 {$\cdot$}
\putt -2 2 {$\cdot$}
\putt -2.5 2.5 {$\cdot$}
}}
}}

\def\ul1cdots{\hbox{
\putt -0.2 -0.2 {\hbox{
\putt 0 0 {$\cdot$}
\putt -1 1 {$\cdot$}
\putt -2 2 {$\cdot$}
}}
}}

\def\dlcdotsconv{\hbox{		%sequence of dots going down left & converging
\putt -0.5 0.85 {$\cdot$}
\putt -0.5 -0.15 {$\cdot$}

\putt -1 0.2 {$\cdot$}
\putt -1 -0.7 {$\cdot$}

\putt -1.5 -0.45 {$\cdot$}
\putt -1.5 -1.05 {$\cdot$}

\putt -2.0 -1.1 {$\cdot$}
\putt -2.0 -1.4 {$\cdot$}

\putt -2.5 -1.6 {$\cdot$}
\putt -2.5 -1.9 {$\cdot$}

\putt -3 -2.25 {$\cdot$}
}}

\def\ulcdotsconv{\hbox{		%sequence of dots going up left & converging
\putt -0.5 -0.85 {$\cdot$}
\putt -0.5 0.15 {$\cdot$}

\putt -1 -0.2 {$\cdot$}
\putt -1 0.7 {$\cdot$}

\putt -1.5 0.45 {$\cdot$}
\putt -1.5 1.05 {$\cdot$}

\putt -2.0 1.1 {$\cdot$}
\putt -2.0 1.4 {$\cdot$}

\putt -2.5 1.6 {$\cdot$}
\putt -2.5 1.9 {$\cdot$}

\putt -3 2.25 {$\cdot$}
}}

\def\tcubenine{\hbox{
		\putt 0 0 {\tcube}
		\putt 1.5 1.5 {\tcube}
		\putt -1.5 1.5 {\tcube}
		\putt 3 3 {\tcube}
		\putt -3 3 {\tcube}
		\putt 0 3 {\tcube}
		\putt 0 6 {\tcube}
		\putt 1.5 4.5 {\tcube}
		\putt -1.5 4.5 {\tcube}
}}

\def\tcubefour{\hbox{
		\putt 0 0 {\tcube}
		\putt 1.5 1.5 {\tcube}
		\putt -1.5 1.5 {\tcube}
		\putt 0 3 {\tcube}
}}



\def\trflap{\hbox{
\point 0 0
\point 1.5 1.5
\point 0 1.5
\point 1.5 3
\tlinep 0 0
\tlinep 0 1.5 
\vline 0 0 1.5
\vline 1.5 1.5 1.5
}}               
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\tlflap{\hbox{
\point 0 0
\point -1.5 1.5
\point 0 1.5
\point -1.5 3
\tlinem 0 0
\tlinem 0 1.5
\vline 0 0 1.5
\vline -1.5 1.5 1.5
}}



\def\trflaps{\hbox{		%small right flap with solid points
\spoint 0 0
\spoint 1.5 1.5
\spoint 0 1.5
\spoint 1.5 3
\tlinep 0 0
\tlinep 0 1.5 
\vline 0 0 1.5
\vline 1.5 1.5 1.5
}}               
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\tlflaps{\hbox{		%small left flap with solid points
\spoint 0 0
\spoint -1.5 1.5
\spoint 0 1.5
\spoint -1.5 3
\tlinem 0 0
\tlinem 0 1.5
\vline 0 0 1.5
\vline -1.5 1.5 1.5
}}

%%%%%%%%%%%%%%
%cdots going down right and angling down
\def\drangdcdots{\hbox{
\putt -0.1 -0.1 {\hbox{
\putt 0 0 {$\cdot$}
\putt 0.5 -0.7 {$\cdot$}
\putt 1 -1.5 {$\cdot$}
\putt 1.5 -2.3 {$\cdot$}
\putt 2 -3.1 {$\cdot$}
\putt 2.5 -3.8 {$\cdot$}
}}
}}
%%%%%%%%%%%%%%%%%%%%%%%%%
%cdots going up right and angling up
\def\urangucdots{\hbox{
\putt 0 0 {$\cdot$}
\putt 0.5 0.7 {$\cdot$}
\putt 1 1.8 {$\cdot$}
\putt 1.5 2.3 {$\cdot$}
\putt 2 3.1 {$\cdot$}
\putt 2.5 3.8 {$\cdot$}
}}

